Learning to reinforcement learn

In recent years deep reinforcement learning (RL) systems have attained superhuman performance in a number of challenging task domains. However, a major limitation of such applications is their demand for massive amounts of training data. A critical present objective is thus to develop deep RL methods that can adapt rapidly to new tasks. In the present work we introduce a novel approach to this challenge, which we refer to as deep meta-reinforcement learning. Previous work has shown that recurrent networks can support meta-learning in a fully supervised context. We extend this approach to the RL setting. What emerges is a system that is trained using one RL algorithm, but whose recurrent dynamics implement a second, quite separate RL procedure. This second, learned RL algorithm can differ from the original one in arbitrary ways. Importantly, because it is learned, it is configured to exploit structure in the training domain. We unpack these points in a series of seven proof-of-concept experiments, each of which examines a key aspect of deep meta-RL. We consider prospects for extending and scaling up the approach, and also point out some potentially important implications for neuroscience.

==> approach.tex <==
\iffalse


\section{Approach}
\label{sec:approach}

All experiments are conducted within a reinforcement learning setting, wherein an agent observes the environment and produces an action in order to maximize cumulative future reward. Our main tasks of consideration are bandits and %finite-horizon tabular% 
Markov decision processes (MDPs), defined by a set of states $S$, discrete actions $A$, and rewards $R$. Agents attempt to maximize total discounted sum of rewards across an entire "episode", composed of $N$ repeated interactions with the MDP (each repetition is termed a "trial") (Figure \ref{fig:archs}).

The architecture consists of a long-short term memory network (LSTM; 48 (Experiments 1-5) or 256 (Experiment 6) cells)(ref). Observations of the environment $o_t$ are either a one-hot vector representing the tabular state, an 84x84 RGB image, or not provided (in the case of bandits). In the experiment using RGB images, a 3-layer encoder was used: two convolutional layers (first layer: 16 8x8 filters applied with stride 4, second layer: 32 4x4 filters with stride 2) followed by a fully connected layer with 256 units and then a ReLU non-linearity (ref Mnih 2013). State information is concatenated with observations relating to past reward $r_t-1$, the last action $a_t-1$ sampled from the policy, and the current time step $t$, and fed as input into the LSTM. The architecture is trained using the Asynchronous Advantage Actor-Critic (A3C) algorithm \cite{mnih2016a3c} which can be considered an actor-critic method that involves learning both a policy $\pi(a_t|s_t;\theta)$ and a value function $V(s_t;\theta_V)$. The policy and value function are computed using linear projections of the LSTM output. There is a softmax output for actions with one unit per action, and a single unit for the value function. The network was unrolled for 20 timesteps (15 for Experiment 3, 160 for Experiment 4, 100 for Experiment 6). Our setup, including the use of entropy regularization, closely follows \cite{mnih2016a3c}. Optimizer. Number of actions. Action repeat. Gradient rescaling for value.

We implemented A3C with 32 threads in experiment 6, but single threaded for all other experiments 1-5 ("LSTM A2C").

The advantage function $A$ is used to estimate the policy gradient which updates model parameters $\theta$ and $\theta_V$:
\begin{equation}
    A(s_t, a_t; \theta_V) = \sum_{i=0}^{k-1} \gamma^i r_{t+i} + \gamma^k V(s_{t+k};\theta_V) - V(s_t;\theta_V).
\end{equation}

% Loss equation, total loss = value est loss + policy loss

% These details can be found in the Appendix. We note that the main model used in 
% our work is recurrent, though, for comparison, we also run a feedforward version of the agent. 

\begin{figure}[ht]
  \centering
    \includegraphics[width=0.65\textwidth]{figures/metaRL_architectures.pdf}
    
    % \subfloat[\scriptsize{LSTM A2C}]{
    % \includegraphics[width=0.15\textwidth]{figures/bandit_arch.png}
    % }
    % \subfloat[\scriptsize{LSTM A3C}]{
    % \includegraphics[width=0.15\textwidth]{figures/harlow_arch.png}
    % }
    % \subfloat[\scriptsize{Nav A3C}]{
    % \includegraphics[width=0.25\textwidth]{figures/nina_arch.png}
    % }
    \caption{ Asynchronous advantage actor-critic with recurrence. In all architectures: observation, reward, last action, and timestep in episode are additional inputs to LSTM; policy ($\pi$) and value function outputs.a) used in experiments 1-5  b)  convolutional-LSTM architecture used in experiment 6 c) stacked LSTM architecture with convolutional encoder used in experiment 6. A2C is single-threaded version, A3C is distributed version.   
    }
    \label{fig:archs}
\end{figure}

%[Thus, the observation $s_t$ may include an image ${\bf x}_t \in \mathbb{R}^{3\times W \times H}$ (where $W$ and $H$ are the width and height of the image), the previous action ${\bf a}_{t-1} \in \mathbb{R}^{N_A}$, and the previous reward $r_{t-1} \in \mathbb{R}$.]

Figure \ref{fig:archs} depicts the advantange actor-critic architectures that we consider, augmented with auxilliary input such as last action, reward, and current time step. For experiment 6, the architecture includes a two-layer convolutional encoder to handle visual input. The agent is trained online, with the value estimate loss and gradient loss, with the value loss weighted according to a parameter $c$ that varies for the different tasks.

\fi

